Tests of light-lepton universality in angular asymmetries of $B^0 \to D^{*-} \ell \nu$ decays

We present the first comprehensive tests of light-lepton universality in the angular distributions of semileptonic $B^0$-meson decays to charged spin-1 charmed mesons. We measure five angular-asymmetry observables as functions of the decay recoil that are sensitive to lepton-universality-violating contributions. We use events where one neutral $B$ is fully reconstructed in $\Upsilon\left(4S\right)\to{}B \overline{B}$ decays in data corresponding to $189~\mathrm{fb}^{-1}$ integrated luminosity from electron-positron collisions collected with the Belle II detector. We find no significant deviation from the standard model expectations.

==> afb_results_table_prl_OLD.tex <==
\begin{table}
  \centering
  \caption{A summary of our measurements of the $\Delta\mathcal{A}$ observables (Obs.) that are sensitive to lepton universality violation, compared to their standard model (SM) expectations. The experimental uncertainties contain both statistical and systematic sources, but are dominated by the statistical uncertainty. An SM expectation of $0\pm0$ indicates a value consistent with zero within machine precision.}
  \label{tab:results_prl}


  % fixe alignm ent of entries without exponent
  \sisetup{table-align-comparator=false, table-align-uncertainty=false, table-align-exponent=true}
  \begin{tabular}{ll
      % siunitx column types for processing uncertainties, exponents with alignment
      S[table-format=2.3+-1.3]
      S[table-format=+4(1)e+1]
    }
    \toprule
    Obs.                     & $w$ bin            & \text{Measurement} & \text{SM}   \\
    \midrule
    $\Delta A_{\mathrm{FB}}$ & $w_\mathrm{low}$   & 0.044+-0.061       & -104(2)e-5  \\
                             & $w_\mathrm{high}$  & -0.16+-0.068       & -1133(9)e-5 \\
                             & $w_\mathrm{incl.}$ & -0.051+-0.043      & -566(6)e-5  \\
    $\Delta S_3$             & $w_\mathrm{low}$   & -0.014+-0.067      & 279(2.)e-6  \\
                             & $w_\mathrm{high}$  & -0.134+-0.068      & 233(8)e-6    \\
                             & $w_\mathrm{incl.}$ & -0.072+-0.046      & 176(6)e-6    \\
    $\Delta S_5$             & $w_\mathrm{low}$   & 0.004+-0.068       & 272(3)e-6  \\
                             & $w_\mathrm{high}$  & -0.063+-0.067      & 107(4)e-5   \\
                             & $w_\mathrm{incl.}$ & -0.028+-0.047      & 49(2)e-5    \\
    $\Delta S_7$             & $w_\mathrm{low}$   & -0.001+-0.066      & 0(0)   \\
                             & $w_\mathrm{high}$  & -0.06+-0.065       & 0(0)   \\
                             & $w_\mathrm{incl.}$ & -0.036+-0.044      & 0(0)   \\
    $\Delta S_9$             & $w_\mathrm{low}$   & 0.003+-0.067       & 0(0)   \\
                             & $w_\mathrm{high}$  & 0.036+-0.067       & 0(0)   \\
                             & $w_\mathrm{incl.}$ & 0.015+-0.046       & 0(0)   \\
    \bottomrule
  \end{tabular}
\end{table}



==> afb_results_table_sm.tex <==
\begin{table}
\centering
\caption{: Full results and total uncertainties from all angular observables along with the standard model expectations.}
\label{tab:results_sm}
\begin{tabular}{llrc}
\toprule
                     Obs. &             $w$ bin &       Measurement &    SM \\
\midrule
      $A_{\mathrm{FB}}^e$ &    $w_\mathrm{low}$ &   $0.149\pm0.045$ &   $\phantom{-}0.272\pm0.005$ \\
                          &   $w_\mathrm{high}$ &   $0.213\pm0.051$ &   $\phantom{-}0.209\pm0.003$ \\
                          &  $w_\mathrm{incl.}$ &   $0.183\pm0.033$ &   $\phantom{-}0.244\pm0.004$ \\
    $A_{\mathrm{FB}}^\mu$ &    $w_\mathrm{low}$ &    $0.248\pm0.040$ &  $\phantom{-}0.271\pm0.005$ \\
                          &   $w_\mathrm{high}$ &   $0.045\pm0.051$ &   $\phantom{-}0.198\pm0.003$ \\
                          &  $w_\mathrm{incl.}$ &   $0.158\pm0.032$ &   $\phantom{-}0.239\pm0.004$ \\
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &    $0.099\pm0.060$ &  $\phantom{l000000}(-1.04\pm0.02)\times 10^{-3}$ \\
                          &   $w_\mathrm{high}$ &  $-0.168\pm0.073$ &   $\phantom{l00000}(-11.33\pm0.09)\times 10^{-3}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.024\pm0.046$ &   $\phantom{l000000}(-5.66\pm0.06)\times 10^{-3}$ \\
                  $S_3^e$ &    $w_\mathrm{low}$ &  $-0.133\pm0.053$ &   $-0.147\pm0.002$ \\
                          &   $w_\mathrm{high}$ &  $-0.016\pm0.053$ &   $-0.063\pm0.002$ \\
                          &  $w_\mathrm{incl.}$ &   $-0.080\pm0.037$ &  $-0.110\pm0.002$ \\
                $S_3^\mu$ &    $w_\mathrm{low}$ &  $-0.159\pm0.048$ &   $-0.147\pm0.002$ \\
                          &   $w_\mathrm{high}$ &  $-0.117\pm0.051$ &   $-0.063\pm0.002$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.142\pm0.034$ &   $-0.110\pm0.002$ \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  $-0.026\pm0.072$ &   $\phantom{00000000}(0.279\pm0.002)\times 10^{-3}$ \\
                          &   $w_\mathrm{high}$ &  $-0.101\pm0.073$ &   $\phantom{00000000}(0.233\pm0.008)\times 10^{-3}$ \\
                          &  $w_\mathrm{incl.}$ &   $-0.062\pm0.050$ &  $\phantom{00000000}(0.176\pm0.005)\times 10^{-3}$ \\
                  $S_5^e$ &    $w_\mathrm{low}$ &   $0.166\pm0.054$ &   $\phantom{-}0.172\pm0.004$ \\
                          &   $w_\mathrm{high}$ &    $0.215\pm0.050$ &  $\phantom{-}0.221\pm0.004$ \\
                          &  $w_\mathrm{incl.}$ &    $0.190\pm0.036$ &  $\phantom{-}0.194\pm0.004$ \\
                $S_5^\mu$ &    $w_\mathrm{low}$ &   $0.146\pm0.049$ &   $\phantom{-}0.172\pm0.004$ \\
                          &   $w_\mathrm{high}$ &    $0.160\pm0.048$ &  $\phantom{-}0.222\pm0.004$ \\
                          &  $w_\mathrm{incl.}$ &   $0.155\pm0.034$ &   $\phantom{-}0.194\pm0.004$ \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &  $-0.019\pm0.073$ &   $\phantom{00000000}(0.272\pm0.003)\times 10^{-3}$ \\
                          &   $w_\mathrm{high}$ &  $-0.055\pm0.069$ &   $\phantom{000000000}(1.07\pm0.04)\phantom{0}\times 10^{-3}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.035\pm0.049$ &   $\phantom{000000000}(0.49\pm0.02)\phantom{0}\times 10^{-3}$ \\
                  $S_7^e$ &    $w_\mathrm{low}$ &  $-0.088\pm0.053$ &     $\phantom{l000}0.0\pm0.0\phantom{00}$ \\
                          &   $w_\mathrm{high}$ &   $0.045\pm0.049$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.018\pm0.035$ &           $\phantom{-}0.0\pm0.0$ \\
                $S_7^\mu$ &    $w_\mathrm{low}$ &   $-0.060\pm0.047$ &           $\phantom{-}0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &   $-0.020\pm0.047$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.043\pm0.033$ &           $\phantom{-}0.0\pm0.0$ \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &   $0.028\pm0.071$ &           $\phantom{-}0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &  $-0.066\pm0.069$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.026\pm0.049$ &           $\phantom{-}0.0\pm0.0$ \\
                  $S_9^e$ &    $w_\mathrm{low}$ &  $-0.035\pm0.054$ &           $\phantom{-}0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &    $0.020\pm0.052$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.004\pm0.036$ &           $\phantom{-}0.0\pm0.0$ \\
                $S_9^\mu$ &    $w_\mathrm{low}$ &  $-0.003\pm0.048$ &           $\phantom{-}0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &    $0.040\pm0.050$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &   $0.016\pm0.034$ &           $\phantom{-}0.0\pm0.0$ \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &   $0.032\pm0.071$ &           $\phantom{-}0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &    $0.020\pm0.072$ &           $\phantom{-}0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &     $0.020\pm0.050$ &           $\phantom{-}0.0\pm0.0$ \\
\bottomrule
\end{tabular}
\end{table}


==> afb_results_table_sm_BACKUP.tex <==
\begin{table}
\centering
\caption{: Full results and total uncertainties from all angular observables (Obs.) along with the standard model expectations (SM).}
\label{tab:results_sm}
\begin{tabular}{llrr}
\toprule
                     Obs. &             $w$ bin &       Measurement &       SM$\phantom{000000}$ \\
\midrule
      $A_{\mathrm{FB}}^e$ &    $w_\mathrm{low}$ &   $0.149\pm0.045$ &   $0.27212\pm0.00456$ \\
                          &   $w_\mathrm{high}$ &   $0.213\pm0.051$ &   $0.20939\pm0.00295$ \\
                          &  $w_\mathrm{incl.}$ &   $0.183\pm0.033$ &   $0.24440\pm0.00366$ \\
    $A_{\mathrm{FB}}^\mu$ &    $w_\mathrm{low}$ &    $0.248\pm0.040$ &  $0.27108\pm0.00454$ \\
                          &   $w_\mathrm{high}$ &   $0.045\pm0.051$ &   $0.19806\pm0.00296$ \\
                          &  $w_\mathrm{incl.}$ &   $0.158\pm0.032$ &   $0.23874\pm0.00365$ \\
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &    $0.099\pm0.060$ &  $-0.00104\pm0.00002$ \\
                          &   $w_\mathrm{high}$ &  $-0.168\pm0.073$ &   $-0.01133\pm0.00009$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.024\pm0.046$ &   $-0.00566\pm0.00006$ \\
                  $S_3^e$ &    $w_\mathrm{low}$ &  $-0.133\pm0.053$ &   $-0.14701\pm0.00190$ \\
                          &   $w_\mathrm{high}$ &  $-0.016\pm0.053$ &   $-0.06280\pm0.00200$ \\
                          &  $w_\mathrm{incl.}$ &   $-0.080\pm0.037$ &  $-0.10980\pm0.00198$ \\
                $S_3^\mu$ &    $w_\mathrm{low}$ &  $-0.159\pm0.048$ &   $-0.14673\pm0.00190$ \\
                          &   $w_\mathrm{high}$ &  $-0.117\pm0.051$ &   $-0.06257\pm0.00200$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.142\pm0.034$ &   $-0.10963\pm0.00198$ \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  $-0.026\pm0.072$ &   $0.00028\pm0.00000$ \\
                          &   $w_\mathrm{high}$ &  $-0.101\pm0.073$ &   $0.00023\pm0.00004$ \\
                          &  $w_\mathrm{incl.}$ &   $-0.062\pm0.050$ &  $0.00018\pm0.00001$ \\
                  $S_5^e$ &    $w_\mathrm{low}$ &   $0.166\pm0.054$ &   $0.17208\pm0.00351$ \\
                          &   $w_\mathrm{high}$ &    $0.215\pm0.050$ &  $0.22067\pm0.00373$ \\
                          &  $w_\mathrm{incl.}$ &    $0.190\pm0.036$ &  $0.19355\pm0.00356$ \\
                $S_5^\mu$ &    $w_\mathrm{low}$ &   $0.146\pm0.049$ &   $0.17235\pm0.00351$ \\
                          &   $w_\mathrm{high}$ &    $0.160\pm0.048$ &  $0.22174\pm0.00369$ \\
                          &  $w_\mathrm{incl.}$ &   $0.155\pm0.034$ &   $0.19405\pm0.00354$ \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &  $-0.019\pm0.073$ &     $0.00027\pm0.00000$ \\
                          &   $w_\mathrm{high}$ &  $-0.055\pm0.069$ &     $0.00107\pm0.00004$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.035\pm0.049$ &     $0.00049\pm0.00002$ \\
                  $S_7^e$ &    $w_\mathrm{low}$ &  $-0.088\pm0.053$ &     $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &   $0.045\pm0.049$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.018\pm0.035$ &           $0.0\pm0.0\phantom{0000}$ \\
                $S_7^\mu$ &    $w_\mathrm{low}$ &   $-0.060\pm0.047$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &   $-0.020\pm0.047$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.043\pm0.033$ &           $0.0\pm0.0\phantom{0000}$ \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &   $0.028\pm0.071$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &  $-0.066\pm0.069$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.026\pm0.049$ &           $0.0\pm0.0\phantom{0000}$ \\
                  $S_9^e$ &    $w_\mathrm{low}$ &  $-0.035\pm0.054$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &    $0.020\pm0.052$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.004\pm0.036$ &           $0.0\pm0.0\phantom{0000}$ \\
                $S_9^\mu$ &    $w_\mathrm{low}$ &  $-0.003\pm0.048$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &    $0.040\pm0.050$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &   $0.016\pm0.034$ &           $0.0\pm0.0\phantom{0000}$ \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &   $0.032\pm0.071$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &   $w_\mathrm{high}$ &    $0.020\pm0.072$ &           $0.0\pm0.0\phantom{0000}$ \\
                          &  $w_\mathrm{incl.}$ &     $0.020\pm0.050$ &           $0.0\pm0.0\phantom{0000}$ \\
\bottomrule
\end{tabular}
\end{table}


==> afb_results_table_sm_OLD.tex <==
\begin{table}[]
  \centering
  \caption{Full results from all angular observables (Obs.) along with the standard model expectations (SM).}
  \label{tab:results_sm}
  \sisetup{
    separate-uncertainty=true, % controls whether uncertainty is given by \pm or in parantheses
    table-alignment-mode=marker, % align on decimal marker
    table-align-uncertainty=true,
    table-align-exponent=true,
    bracket-ambiguous-numbers=false, % if true, adds parentheses around separate uncertainties with exponent, breaks formatting
  }
  \begin{tabular}{ll
      % siunivvvvvvvtx column types for processing uncertainties, exponents with alignment
      % HACK: I use zero-decimal-to-integer=true and 0.0 float uncertainties, because with integer 0 uncertainties siunitx drops them
      S[table-format=+1.3+-1.3]
      % in the format I set the uncertainty digits to 5 instead of 3 in order to increase the distance of the exponent in order to reduce ambiguouity with `bracket-ambiguous-numbers=false`
      S[table-format=+2.3(1.5)e+1]
    }
    \toprule
    Obs.                     & $w$ bin            & \text{Measurement} & \text{SM}      \\
    \midrule

    $A_{\mathrm{FB}}^e$      & $w_\mathrm{low}$   & 0.192+-0.045       & 0.272(0.004)  \\
                             & $w_\mathrm{high}$  & 0.228+-0.049       & 0.209(0.003)  \\
                             & $w_\mathrm{incl.}$ & 0.211+-0.03        & 0.244(0.004)  \\
    $A_{\mathrm{FB}}^\mu$    & $w_\mathrm{low}$   & 0.236+-0.042       & 0.271(0.005)  \\
                             & $w_\mathrm{high}$  & 0.068+-0.047       & 0.198(0.003)  \\
                             & $w_\mathrm{incl.}$ & 0.16+-0.031        & 0.239(0.004)  \\
    $\Delta A_{\mathrm{FB}}$ & $w_\mathrm{low}$   & 0.044+-0.061       & -1.04(0.02)e-3     \\
                             & $w_\mathrm{high}$  & -0.16+-0.068       & -11.33(0.09)e-3    \\
                             & $w_\mathrm{incl.}$ & -0.051+-0.043      & -5.66(0.06)e-3     \\
    $S_3^e$                  & $w_\mathrm{low}$   & -0.156+-0.048      & -0.147(0.002) \\
                             & $w_\mathrm{high}$  & -0.004+-0.048      & -0.063(.002)  \\
                             & $w_\mathrm{incl.}$ & -0.087+-0.032      & -0.110(.002) \\
    $S_3^\mu$                & $w_\mathrm{low}$   & -0.17+-0.046       & -0.147(0.002) \\
                             & $w_\mathrm{high}$  & -0.138+-0.048      & -0.063(0.002)  \\
                             & $w_\mathrm{incl.}$ & -0.159+-0.033      & -0.111(0.002) \\
    $\Delta S_3$             & $w_\mathrm{low}$   & -0.014+-0.067      & 2.79(0.02)e-4  \\
                             & $w_\mathrm{high}$  & -0.134+-0.068      & 2.33(0.08)e-4    \\
                             & $w_\mathrm{incl.}$ & -0.072+-0.046      & 1.76(0.06)e-4    \\
    $S_5^e$                  & $w_\mathrm{low}$   & 0.152+-0.05        & 0.172(0.004)  \\
                             & $w_\mathrm{high}$  & 0.225+-0.048       & 0.221(0.004)  \\
                             & $w_\mathrm{incl.}$ & 0.187+-0.035       & 0.194(0.004)  \\
    $S_5^\mu$                & $w_\mathrm{low}$   & 0.156+-0.046       & 0.172(0.004)  \\
                             & $w_\mathrm{high}$  & 0.162+-0.047       & 0.222(0.004)  \\
                             & $w_\mathrm{incl.}$ & 0.159+-0.031       & 0.194(0.004)  \\
    $\Delta S_5$             & $w_\mathrm{low}$   & 0.004+-0.068       & 2.72(0.03)e-4  \\
                             & $w_\mathrm{high}$  & -0.063+-0.067      & 10.7(0.4)e-4   \\
                             & $w_\mathrm{incl.}$ & -0.028+-0.047      & 4.93(0.21)e-4    \\
    $S_7^e$                  & $w_\mathrm{low}$   & -0.082+-0.048      & 0(0)      \\
                             & $w_\mathrm{high}$  & 0.026+-0.046       & 0(0)      \\
                             & $w_\mathrm{incl.}$ & -0.024+-0.032      & 0(0)      \\
    $S_7^\mu$                & $w_\mathrm{low}$   & -0.083+-0.045      & 0(0)      \\
                             & $w_\mathrm{high}$  & -0.033+-0.046      & 0(0)      \\
                             & $w_\mathrm{incl.}$ & -0.06+-0.031       & 0(0)      \\
    $\Delta S_7$             & $w_\mathrm{low}$   & -0.001+-0.066      & 0(0)      \\
                             & $w_\mathrm{high}$  & -0.06+-0.065       & 0(0)      \\
                             & $w_\mathrm{incl.}$ & -0.036+-0.044      & 0(0)      \\
    $S_9^e$                  & $w_\mathrm{low}$   & -0.026+-0.049      & 0(0)      \\
                             & $w_\mathrm{high}$  & 0.01+-0.048        & 0(0)      \\
                             & $w_\mathrm{incl.}$ & -0.005+-0.034      & 0(0)      \\
    $S_9^\mu$                & $w_\mathrm{low}$   & -0.023+-0.045      & 0(0)      \\
                             & $w_\mathrm{high}$  & 0.046+-0.047       & 0(0)      \\
                             & $w_\mathrm{incl.}$ & 0.01+-0.032        & 0(0)      \\
    $\Delta S_9$             & $w_\mathrm{low}$   & 0.003+-0.067       & 0(0)      \\
                             & $w_\mathrm{high}$  & 0.036+-0.067       & 0(0)      \\
                             & $w_\mathrm{incl.}$ & 0.015+-0.046       & 0(0)      \\
    \bottomrule
  \end{tabular}
\end{table}


==> afb_syst_table_prl.tex <==
\begin{table}
\centering
\caption{}
\label{tab:systematics_prl}
\begin{tabular}{llccccc}
\toprule
                     Obs. &             $w$ bin &  Total &  Stat. &  MC stat. &    LID &  $\pi_{\textrm{slow}}$ \\
\midrule
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &  0.060 &  0.056 &     0.020 &  0.004 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.073 &  0.068 &     0.024 &  0.004 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.046 &  0.043 &     0.015 &  0.004 &                  0.001 \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  0.072 &  0.068 &     0.024 &  0.001 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.073 &  0.069 &     0.025 &  0.001 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.050 &  0.047 &     0.017 &  0.001 &                  0.000 \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &  0.073 &  0.068 &     0.024 &  0.001 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.069 &  0.065 &     0.023 &  0.001 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.049 &  0.046 &     0.016 &  0.001 &                  0.000 \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &  0.071 &  0.067 &     0.023 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.069 &  0.065 &     0.022 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.049 &  0.046 &     0.016 &  0.000 &                  0.000 \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &  0.071 &  0.067 &     0.024 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.072 &  0.068 &     0.024 &  0.001 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.050 &  0.047 &     0.017 &  0.000 &                  0.000 \\
\bottomrule
\end{tabular}
\end{table}


==> afb_syst_table_sm.tex <==
\begin{table}
\centering
\caption{Summary of the experimental uncertainties for all angular observables (Obs.) classified by relevant source: sample size (Stat.), MC sample size (MC stat.), lepton ID (LID), and slow-pion efficiency ($\pi_{	\textrm{slow}}$).}
\label{tab:systematics_sm}
\begin{tabular}{llccccc}
\toprule
                     Obs. &             $w$ bin &  Total &  Stat. &  MC stat. &    LID &  $\pi_{\textrm{slow}}$ \\
\midrule
      $A_{\mathrm{FB}}^e$ &    $w_\mathrm{low}$ &  0.045 &  0.042 &     0.015 &  0.004 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.051 &  0.048 &     0.017 &  0.004 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.033 &  0.031 &     0.011 &  0.004 &                  0.001 \\
    $A_{\mathrm{FB}}^\mu$ &    $w_\mathrm{low}$ &  0.040 &  0.038 &     0.013 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.051 &  0.048 &     0.016 &  0.002 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.032 &  0.030 &     0.010 &  0.001 &                  0.001 \\
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &  0.060 &  0.056 &     0.020 &  0.004 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.073 &  0.068 &     0.024 &  0.004 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.046 &  0.043 &     0.015 &  0.004 &                  0.001 \\
                  $S_3^e$ &    $w_\mathrm{low}$ &  0.053 &  0.050 &     0.018 &  $<0.001\phantom{0~~}$ &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.053 &  0.049 &     0.018 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.037 &  0.034 &     0.012 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                $S_3^\mu$ &    $w_\mathrm{low}$ &  0.048 &  0.045 &     0.016 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.051 &  0.048 &     0.016 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.034 &  0.032 &     0.011 &  0.001 &                  $<0.001\phantom{0~~}$ \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  0.072 &  0.068 &     0.024 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.073 &  0.069 &     0.025 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.050 &  0.047 &     0.017 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                  $S_5^e$ &    $w_\mathrm{low}$ &  0.054 &  0.051 &     0.018 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.050 &  0.047 &     0.017 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.036 &  0.034 &     0.012 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                $S_5^\mu$ &    $w_\mathrm{low}$ &  0.049 &  0.046 &     0.016 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.048 &  0.045 &     0.016 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.034 &  0.032 &     0.011 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &  0.073 &  0.068 &     0.024 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.069 &  0.065 &     0.023 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.049 &  0.046 &     0.016 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                  $S_7^e$ &    $w_\mathrm{low}$ &  0.053 &  0.050 &     0.018 &  0.001 &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.049 &  0.046 &     0.017 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.035 &  0.033 &     0.012 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                $S_7^\mu$ &    $w_\mathrm{low}$ &  0.047 &  0.045 &     0.015 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.047 &  0.045 &     0.015 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.033 &  0.031 &     0.011 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &  0.071 &  0.067 &     0.023 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.069 &  0.065 &     0.022 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.049 &  0.046 &     0.016 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                  $S_9^e$ &    $w_\mathrm{low}$ &  0.054 &  0.050 &     0.018 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.052 &  0.049 &     0.018 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &  $w_\mathrm{incl.}$ &  0.036 &  0.034 &     0.012 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                $S_9^\mu$ &    $w_\mathrm{low}$ &  0.048 &  0.046 &     0.016 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.050 &  0.047 &     0.016 &  $<0.001\phantom{0~~}$ &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.034 &  0.032 &     0.011 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &  0.071 &  0.067 &     0.024 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
                          &   $w_\mathrm{high}$ &  0.072 &  0.068 &     0.024 &  0.001 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.050 &  0.047 &     0.017 &  $<0.001\phantom{0~~}$ &                  $<0.001\phantom{0~~}$ \\
\bottomrule
\end{tabular}
\end{table}


==> afb_syst_table_sm_OLD.tex <==
\begin{table}
  \centering
  \caption{A breakdown of the experimental uncertainties for all angular observables (Obs.) by relevant source: sample size (Stat.), MC sample size (MC stat.), lepton ID (LID), and slow pion efficiency ($\pi_{\textrm{slow}}$).}
  \label{tab:systematics_sm}
  \sisetup{table-format=1.3}
  \begin{tabular}{llSSSSS}
    \toprule
    Obs.                     & $w$ bin            & \text{Total} & \text{Stat.} & \text{MC stat.} & \text{LID} & $\pi_{\textrm{slow}}$ \\
    \midrule
    $A_{\mathrm{FB}}^e$      & $w_\mathrm{low}$  & 
     0.049 &  0.047 &     0.013 &  0.004 &                  0.001 \\
                           &   $w_\mathrm{high}$ &  0.049 &  0.047 &     0.013 &  0.004 &                  0.001 \\    
                          &  $w_\mathrm{incl.}$ &  0.031 &  0.029 &     0.008 &  0.003 &                  0.001 \\
    $A_{\mathrm{FB}}^\mu$ &    $w_\mathrm{low}$ &  0.042 &  0.041 &     0.010 &  0.001 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.048 &  0.046 &     0.012 &  0.002 &                  0.001 \\
                          &  $w_\mathrm{incl.}$ &  0.031 &  0.030 &     0.008 &  0.001 &                  0.001 \\
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &  0.062 &  0.060 &     0.015 &  0.004 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.068 &  0.066 &     0.018 &  0.004 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.043 &  0.042 &     0.011 &  0.004 &                  0.001 \\
                  $S_3^e$ &    $w_\mathrm{low}$ &  0.048 &  0.046 &     0.013 &  0.000 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.049 &  0.047 &     0.014 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.033 &  0.031 &     0.009 &  0.000 &                  0.000 \\
                $S_3^\mu$ &    $w_\mathrm{low}$ &  0.046 &  0.045 &     0.012 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.048 &  0.046 &     0.012 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.033 &  0.032 &     0.008 &  0.000 &                  0.000 \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  0.067 &  0.065 &     0.018 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.068 &  0.066 &     0.018 &  0.001 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.046 &  0.044 &     0.012 &  0.001 &                  0.000 \\
                  $S_5^e$ &    $w_\mathrm{low}$ &  0.051 &  0.049 &     0.014 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.048 &  0.047 &     0.013 &  0.001 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.035 &  0.034 &     0.009 &  0.001 &                  0.000 \\
                $S_5^\mu$ &    $w_\mathrm{low}$ &  0.046 &  0.045 &     0.012 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.047 &  0.045 &     0.012 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.031 &  0.030 &     0.008 &  0.000 &                  0.000 \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &  0.069 &  0.066 &     0.018 &  0.001 &                  0.001 \\
                          &   $w_\mathrm{high}$ &  0.067 &  0.065 &     0.017 &  0.001 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.047 &  0.045 &     0.012 &  0.001 &                  0.000 \\
                  $S_7^e$ &    $w_\mathrm{low}$ &  0.048 &  0.046 &     0.014 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.047 &  0.045 &     0.013 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.032 &  0.030 &     0.009 &  0.000 &                  0.000 \\
                $S_7^\mu$ &    $w_\mathrm{low}$ &  0.045 &  0.044 &     0.012 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.046 &  0.044 &     0.012 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.031 &  0.030 &     0.008 &  0.000 &                  0.000 \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &  0.066 &  0.063 &     0.018 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.066 &  0.063 &     0.017 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.045 &  0.043 &     0.012 &  0.000 &                  0.000 \\
                  $S_9^e$ &    $w_\mathrm{low}$ &  0.050 &  0.048 &     0.014 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.049 &  0.047 &     0.013 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.034 &  0.033 &     0.009 &  0.000 &                  0.000 \\
                $S_9^\mu$ &    $w_\mathrm{low}$ &  0.045 &  0.044 &     0.012 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.048 &  0.046 &     0.012 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.032 &  0.031 &     0.008 &  0.000 &                  0.000 \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &  0.067 &  0.065 &     0.018 &  0.000 &                  0.000 \\
                          &   $w_\mathrm{high}$ &  0.068 &  0.065 &     0.018 &  0.000 &                  0.000 \\
                          &  $w_\mathrm{incl.}$ &  0.047 &  0.045 &     0.012 &  0.000 &                  0.000 \\
    \bottomrule
  \end{tabular}
\end{table}


==> belle2sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers.
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%% \num conflicts with siunitx
% \def\num        {\ensuremath{\nu_\mu}\xspace}
% \def\numb       {\ensuremath{\nub_\mu}\xspace}
% \def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


==> material.tex <==
% INCLUDE ALL FIGURES AND NUMBERS THAT SHOULD BE APPROVED FOR PUBLIC PRESENTATION IN THIS FILE.


==> pub029.tex <==
%%% Paper:    B0 to D*- l+ nu lepton universality
%%% Journal:  Physical Review Letters
%%% Contacts: M. Eliachevitch, M. Hedges, P. Lewis, F. Bernlochner
%%% ====================================================================
%%% Use \input{pub029} to insert this material into your latex file.
\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instChula}{Chulalongkorn University, Bangkok 10330, Thailand}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instRomaENEA}{ENEA Casaccia, I-00123 Roma, Italy}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\newcommand{\instMainz}{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instHeidelberg}{Heidelberg University, 68131 Mannheim, Germany}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007, China}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081, China}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011, U.S.A.}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instJLU}{Jilin University, Changchun 130012, China}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNNU}{Nanjing Normal University, Nanjing 210023, China}
\newcommand{\instNankai}{Nankai University, Tianjin 300071, China}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instKyiv}{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\newcommand{\instSEU}{Southeast University, Nanjing 211189, China}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419, South Korea}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instManitoba}{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007, India}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instUppsala}{Uppsala University, SE-751 05 Uppsala, Sweden}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
\newcommand{\instZZU}{Zhengzhou University, Zhengzhou 450001, China}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instYerevan}
\affiliation{\instGoettingen}
%%%\affiliation{\instBeihang}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
%%%\affiliation{\instChiba}
%%%\affiliation{\instChonnam}
%%%\affiliation{\instChula}
\affiliation{\instCAU}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instRomaENEA}
%%%\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instMainz}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
%%%\affiliation{\instHeidelberg}
\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
%%%\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instISU}
\affiliation{\instJAEA}
%%%\affiliation{\instJLU}
\affiliation{\instKarlsruhe}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyotoU}
%%%\affiliation{\instKyungpook}
\affiliation{\instLNNU}
\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaIAR}
\affiliation{\instNagoyaKMI}
%%%\affiliation{\instNNU}
%%%\affiliation{\instNankai}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
%%%\affiliation{\instMPGHLL}
%%%\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instSeoul}
\affiliation{\instShandong}
\affiliation{\instKyiv}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instSEU}
\affiliation{\instLjubljanaJSI}
%%%\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
%%%\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
%%%\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
%%%\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instManitoba}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
%%%\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instUppsala}
\affiliation{\instVPI}
\affiliation{\instWayneState}
%%%\affiliation{\instXavier}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
%%%\affiliation{\instZZU}
% \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
  \author{K.~Adamczyk}\affiliation{\instLjubljanaJSI} % 2239
  \author{L.~Aggarwal}\affiliation{\instPanjab} % 10083
% \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
% \author{H.~Ahmed}\affiliation{\instXavier} % 11323
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
% \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{N.~Anh~Ky}\affiliation{\instIOP} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{M.~Aversano}\affiliation{\instNagoya} % 7363
% \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instIPHC} % 5623
% \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{H.~Bae}\affiliation{\instUTokyo} % 10863
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
% \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
% \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
% \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{M.~Bauer}\affiliation{\instKarlsruhe} % 9863
  \author{A.~Baur}\affiliation{\instDESY} % 5683
  \author{A.~Beaubien}\affiliation{\instVictoria} % 6683
% \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{F.~Becherer}\affiliation{\instDESY} % 21623
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
% \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{V.~Bertacchi}\affiliation{\instCPPM} % 2212
  \author{M.~Bertemes}\affiliation{\instBNL} % 2595
  \author{E.~Bertholet}\affiliation{\instTelAviv} % 13163
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
% \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
% \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{D.~Bodrov}\affiliation{\instSoochow}\affiliation{\instHSE} % 9643
  \author{A.~Bolz}\affiliation{\instDESY} % 15403
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
% \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{J.~Borah}\affiliation{\instIITGuwahati} % 7083
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
% \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instDESY} % 2099
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
  \author{J.~Cerasoli}\affiliation{\instIPHC} % 20746
% \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instDESY} % 2208
  \author{P.~Cheema}\affiliation{\instSydney} % 15264
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
% \author{C.~Chen}\affiliation{\instISU} % 12803
% \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
% \author{Y.~Q.~Chen}\affiliation{\instJLU} % 16264
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instBINP} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
% \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instCAU} % 2364
  \author{S.~Choudhury}\affiliation{\instISU}\affiliation{\instKEK} % 2206
% \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{J.~Cochran}\affiliation{\instISU} % 12604
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
  \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
% \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % 2254
  \author{S.~Das}\affiliation{\instMNITJaipur} % 9163
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{S.~A.~De~La~Motte}\affiliation{\instAdelaide} % 2128
% \author{G.~de~Marino}\affiliation{\instLjubljanaUniLJ} % 8364
  \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
  \author{M.~De~Nuccio}\affiliation{\instUBC} % 2610
  \author{G.~De~Pietro}\affiliation{\instKarlsruhe} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
% \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
% \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % 9465
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instITAR} % 2215
  \author{M.~Dorigo}\affiliation{\instTriesteINFN} % 12543
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dreyer}\affiliation{\instDESY} % 12823
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
% \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % 5563
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{P.~Feichtinger}\affiliation{\instHEPHYVienna} % 9843
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{T.~Fillinger}\affiliation{\instKEK} % 9803
  \author{C.~Finck}\affiliation{\instIPHC} % 15803
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
% \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
% \author{K.~Flood}\affiliation{\instHawaii} % 12103
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
% \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{A.~Gabrielli}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13523
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instDESY} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
  \author{R.~Garg}\affiliation{\instCMU} % 2213
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{G.~Gaudino}\affiliation{\instNapoliINFN} % 16563
  \author{V.~Gaur}\affiliation{\instUPES} % 2413
  \author{A.~Gaz}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2181
% \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
  \author{G.~Ghevondyan}\affiliation{\instYerevan} % 9445
  \author{D.~Ghosh}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 11923
  \author{H.~Ghumaryan}\affiliation{\instYerevan} % 19543
  \author{G.~Giakoustidis}\affiliation{\instBonn} % 13723
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
% \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{O.~Gogota}\affiliation{\instKyiv} % 2334
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
% \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instNovaGorica}\affiliation{\instLjubljanaJSI} % 3703
% \author{G.~Gong}\affiliation{\instUSTC} % 2727
% \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
% \author{M.~Graf-Schreiber}\affiliation{\instDESY} % 2730
% \author{T.~Grammatico}\affiliation{\instVictoria} % 20623
  \author{S.~Granderath}\affiliation{\instBonn} % 8383
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Z.~Gruberov\'{a}}\affiliation{\instPrague} % 8824
  \author{T.~Gu}\affiliation{\instPittsburgh} % 14283
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % 10504
% \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
  \author{S.~Halder}\affiliation{\instTata} % 4743
  \author{Y.~Han}\affiliation{\instDESY} % 19663
% \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
% \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{S.~Hazra}\affiliation{\instTata} % 7663
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~T.~Hedges}\affiliation{\instBonn} % 2265
  \author{A.~Heidelbach}\affiliation{\instKarlsruhe} % 16923
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instDESY} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
% \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
  \author{P.~Horak}\affiliation{\instHEPHYVienna} % 13583
% \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
% \author{T.~Humair}\affiliation{\instMPP} % 10643
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI}\affiliation{\instKEK} % 2446
  \author{K.~Inami}\affiliation{\instNagoya}\affiliation{\instKEK} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % 12223
% \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{S.~Ito}\affiliation{\instKEK} % 17463
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % 2360
% \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
% \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
  \author{Q.~P.~Ji}\affiliation{\instHNU} % 16243
  \author{S.~Jia}\affiliation{\instSEU} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
  \author{A.~Johnson}\affiliation{\instIITMadras} % 16143
% \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{H.~Junkerkalefeld}\affiliation{\instBonn} % 12963
% \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
% \author{M.~Kaleta}\affiliation{\instKrakow} % 5603
% \author{D.~Kalita}\affiliation{\instIITGuwahati} % 2220
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % 7344
  \author{J.~Kandra}\affiliation{\instPadovaINFN} % 2541
  \author{K.~H.~Kang}\affiliation{\instIPMU} % 2283
% \author{S.~Kang}\affiliation{\instISU} % 12683
% \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
% \author{R.~Karl}\affiliation{\instDESY} % 10923
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
% \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
% \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{F.~Keil}\affiliation{\instMainz} % 19523
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{K.-H.~Kim}\affiliation{\instKISTI} % 2118
% \author{K.~Kim}\affiliation{\instKoreaUnivKU} % 2409
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % 2403
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
% \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
% \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{K.~Kojima}\affiliation{\instNagoya} % 6363
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % 4185
  \author{S.~Korpar}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % 3884
  \author{R.~Kowalewski}\affiliation{\instVictoria} % 2293
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
% \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
% \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
% \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
% \author{Y.~Kulii}\affiliation{\instLMU} % 9823
% \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
  \author{M.~Kumar}\affiliation{\instIISER} % 2744
% \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instMississippi} % 2257
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
% \author{S.~Kurz}\affiliation{\instDESY} % 9363
% \author{A.~Kusudo}\affiliation{\instNaraWu} % 14623
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
  \author{Y.-T.~Lai}\affiliation{\instKEK} % 2066
% \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{T.~Lam}\affiliation{\instVPI} % 2729
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{M.~Laurenza}\affiliation{\instUppsala} % 10223
% \author{K.~Lautenbach}\affiliation{\instCPPM} % 2102
% \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{R.~Leboucher}\affiliation{\instCPPM} % 14083
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
% \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
  \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{D.~Levit}\affiliation{\instKEK} % 2507
  \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
% \author{S.~X.~Li}\affiliation{\instFudan} % 2377
  \author{Y.~Li}\affiliation{\instFudan} % 8083
% \author{Y.~B.~Li}\affiliation{\instFudan} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
% \author{K.~Lieret}\affiliation{\instLMU} % 2268
% \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
% \author{Y.-R.~Lin}\affiliation{\instNTUTaiwan} % 9323
% \author{Z.~Liptak}\affiliation{\instHiroshima} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
% \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{Z.~Q.~Liu}\affiliation{\instShandong} % 11303
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instManitoba} % 2396
% \author{A.~Lozar}\affiliation{\instLjubljanaJSI} % 12423
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
  \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~Lyu}\affiliation{\instBonn} % 12484
  \author{Y.~Ma}\affiliation{\instRIKENMSL} % 16883
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~P.~Maharana}\affiliation{\instIITHyderabad} % 19083
  \author{R.~Maiti}\affiliation{\instHEPHYVienna} % 12043
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{G.~Mancinelli}\affiliation{\instCPPM} % 20743
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
  \author{A.~C.~Manthei}\affiliation{\instBonn} % 15023
  \author{M.~Mantovano}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 19783
  \author{D.~Marcantonio}\affiliation{\instMelbourne} % 11163
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{L.~Martel}\affiliation{\instIPHC} % 13503
  \author{C.~Martellini}\affiliation{\instRomaTreINFN} % 16983
  \author{A.~Martini}\affiliation{\instDESY} % 2336
  \author{T.~Martinov}\affiliation{\instDESY} % 19463
  \author{L.~Massaccesi}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 16323
  \author{M.~Masuda}\affiliation{\instRCNP}\affiliation{\instEri} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
% \author{K.~Matsuoka}\affiliation{\instKEK}\affiliation{\instNagoya} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % 2351
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % 9763
  \author{J.~A.~McKenna}\affiliation{\instUBC} % 2392
% \author{J.~McNeil}\affiliation{\instFlorida} % 2382
% \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{R.~Mehta}\affiliation{\instTata} % 15203
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
  \author{F.~Metzner}\affiliation{\instBonn} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{M.~Mirra}\affiliation{\instNapoliINFN} % 14744
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % 2327
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
% \author{H.~Miyata}\affiliation{\instNiigata} % 2071
% \author{R.~Mizuk}\affiliation{\instHSE}\affiliation{\instIJCLab} % 2483
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{N.~Molina-Gonzalez}\affiliation{\instCinvestavIPN} % 8004
  \author{S.~Mondal}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 19743
  \author{S.~Moneta}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 13303
% \author{H.~Moon}\affiliation{\instKoreaUnivKU} % 2304
% \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
% \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
% \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
% \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % 2554
% \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{Y.~Nakazawa}\affiliation{\instKEK} % 17383
  \author{A.~Narimani~Charan}\affiliation{\instDESY} % 10143
  \author{M.~Naruki}\affiliation{\instKyotoU} % 4583
% \author{D.~Narwal}\affiliation{\instIITGuwahati} % 7223
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % 9464
% \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
% \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
% \author{M.~Niiyama}\affiliation{\instKSU} % 2063
% \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNiigata} % 2571
% \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
% \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
% \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
% \author{S.~L.~Olsen}\affiliation{\instCAU} % 4563
% \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
% \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
  \author{P.~Oskin}\affiliation{\instIJCLab} % 9623
  \author{F.~Otani}\affiliation{\instUTokyo} % 16244
% \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instHSE} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE} % 2188
  \author{A.~Paladino}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2435
% \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{K.~Parham}\affiliation{\instDuke} % 10684
% \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{S.-H.~Park}\affiliation{\instKEK} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
% \author{A.~Pathak}\affiliation{\instLouisville} % 8723
  \author{S.~Patra}\affiliation{\instLouisville} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
  \author{F.~Pham}\affiliation{\instMelbourne} % 2963
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
% \author{G.~Pinna~Angioni}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 13363
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{T.~Podobnik}\affiliation{\instLjubljanaJSI} % 11223
  \author{S.~Pokharel}\affiliation{\instMississippi} % 12283
% \author{L.~Polat}\affiliation{\instCPPM} % 9783
% \author{V.~Popov}\affiliation{\instTelAviv}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instKEK} % 2726
  \author{S.~Prell}\affiliation{\instISU} % 12743
  \author{E.~Prencipe}\affiliation{\instGiessen} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{H.~Purwar}\affiliation{\instHawaii} % 12363
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instHEPHYVienna} % 7383
  \author{G.~Raeuber}\affiliation{\instHEPHYVienna} % 18143
  \author{S.~Raiz}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13003
% \author{A.~Ramirez~Morales}\affiliation{\instKyungpook} % 13724
% \author{N.~Rauls}\affiliation{\instGoettingen} % 11603
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
% \author{M.~Ritter}\affiliation{\instLMU} % 2580
% \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
% \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
% \author{P.~Rocchetti}\affiliation{\instMelbourne} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{M.~Roehrken}\affiliation{\instDESY} % 11883
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
% \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instTriesteINFN} % 2965
% \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
  \author{D.~Sahoo}\affiliation{\instISU} % 2110
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
% \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
% \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{Y.~Sato}\affiliation{\instKEK} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instUppsala} % 2518
  \author{C.~Schmitt}\affiliation{\instLMU}\affiliation{\instMPP} % 15063
% \author{J.~Schmitz}\affiliation{\instBonn} % 12863
  \author{M.~Schnepf}\affiliation{\instKarlsruhe} % 15683
% \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
% \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
% \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
% \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
% \author{M.~Schwickardi}\affiliation{\instGoettingen} % 14743
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaTreINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{W.~Shan}\affiliation{\instHUNNU} % 11943
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % 11584
% \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instFudan} % 2464
  \author{X.~D.~Shi}\affiliation{\instKEK} % 18843
% \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{T.~Shillington}\affiliation{\instMcGill} % 7983
% \author{T.~Shimasaki}\affiliation{\instUTokyo} % 16263
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{D.~Shtol}\affiliation{\instBINP}\affiliation{\instNSU} % 9223
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instHawaii} % 2419
  \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
  \author{J.~Skorupa}\affiliation{\instMPP} % 12523
% \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{M.~Sobotzik}\affiliation{\instMainz} % 8604
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
% \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instBINP} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{P.~Stavroulakis}\affiliation{\instIPHC} % 20643
  \author{S.~Stefkova}\affiliation{\instKarlsruhe} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
% \author{J.~Stypula}\affiliation{\instKrakow} % 2368
% \author{Y.~Sue}\affiliation{\instNagoya} % 2085
% \author{R.~Sugiura}\affiliation{\instUTokyo} % 4644
  \author{M.~Sumihama}\affiliation{\instRCNP}\affiliation{\instGifu} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNaraWu} % 2583
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
% \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
% \author{M.~Tabata}\affiliation{\instChiba} % 2986
  \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
% \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
% \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
% \author{Y.~Tao}\affiliation{\instFlorida} % 2362
  \author{F.~Tenchini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2546
  \author{A.~Thaller}\affiliation{\instCPPM} % 16044
  \author{O.~Tittel}\affiliation{\instMPP} % 8663
  \author{R.~Tiwary}\affiliation{\instTata} % 10403
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{N.~Toutounji}\affiliation{\instSydney} % 2263
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
  \author{I.~Tsaklidis}\affiliation{\instBonn} % 13443
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{Y.~Uematsu}\affiliation{\instUTokyo} % 5883
% \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{K.~Uno}\affiliation{\instNiigata} % 14963
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instUTokyo}\affiliation{\instSOKENDAI} % 2317
% \author{Y.~V.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instMcGill} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{M.~Veronesi}\affiliation{\instISU} % 20723
% \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{V.~S.~Vismaya}\affiliation{\instIITHyderabad} % 16063
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vobbilisetti}\affiliation{\instIJCLab} % 7364
  \author{R.~Volpe}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 20183
% \author{V.~Vorobyev}\affiliation{\instBINP} % 2298
% \author{A.~Vossen}\affiliation{\instDuke} % 2249
  \author{B.~Wach}\affiliation{\instMPP} % 8203
  \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{M.~Wakai}\affiliation{\instUBC} % 3583
% \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{S.~Wallner}\affiliation{\instMPP} % 20363
% \author{K.~Wan}\affiliation{\instUTokyo} % 2591
% \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
% \author{B.~Wang}\affiliation{\instMPP} % 2569
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{E.~Wang}\affiliation{\instPittsburgh} % 10983
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
% \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{Z.~Wang}\affiliation{\instUTokyo} % 15743
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instYonsei} % 6843
% \author{J.~Webb}\affiliation{\instMelbourne} % 2423
% \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
% \author{O.~Werbycka}\affiliation{\instTriesteINFN} % 6123
  \author{C.~Wessel}\affiliation{\instDESY} % 2100
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % 2604
% \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
% \author{H.~Windel}\affiliation{\instMPP} % 2081
% \author{E.~Won}\affiliation{\instKoreaUnivKU} % 2410
% \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
% \author{Y.~Xie}\affiliation{\instShandong} % 20383
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % 2374
% \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % 2365
% \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{K.~Yoshihara}\affiliation{\instNagoya} % 12663
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
% \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2529
% \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
% \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Y.~Zhang}\affiliation{\instFudan} % 3303
% \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{J.~S.~Zhou}\affiliation{\instFudan} % 12463
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI}\affiliation{\instNagoyaIAR} % 7323
% \author{X.~Y.~Zhou}\affiliation{\instLNNU} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2387
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k}\affiliation{\instPrague} % 13403
\collaboration{The Belle II Collaboration}


==> results_table.tex <==
\begin{table}
\centering
\caption{Exported from plotting script. Needs to be cleaned up.}
\label{tab:results}
\begin{tabular}{llll}
\toprule
               observable &             $w$ bin &       Measurement &                     SM \\
\midrule
 $\Delta A_{\mathrm{FB}}$ &    $w_\mathrm{low}$ &   $0.044\pm0.061$ &  $-0.001042\pm2.1e-05$ \\
                          &   $w_\mathrm{high}$ &   $-0.16\pm0.068$ &    $-0.011333\pm9e-05$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.051\pm0.042$ &  $-0.005659\pm6.5e-05$ \\
             $\Delta S_3$ &    $w_\mathrm{low}$ &  $-0.014\pm0.067$ &     $0.000279\pm2e-06$ \\
                          &   $w_\mathrm{high}$ &  $-0.134\pm0.068$ &     $0.000233\pm8e-06$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.072\pm0.046$ &     $0.000176\pm6e-06$ \\
             $\Delta S_5$ &    $w_\mathrm{low}$ &   $0.004\pm0.068$ &     $0.000272\pm3e-06$ \\
                          &   $w_\mathrm{high}$ &  $-0.063\pm0.067$ &     $0.001072\pm4e-05$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.028\pm0.047$ &   $0.000493\pm2.1e-05$ \\
             $\Delta S_7$ &    $w_\mathrm{low}$ &  $-0.001\pm0.066$ &            $0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &   $-0.06\pm0.065$ &            $0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &  $-0.036\pm0.044$ &            $0.0\pm0.0$ \\
             $\Delta S_9$ &    $w_\mathrm{low}$ &   $0.003\pm0.067$ &            $0.0\pm0.0$ \\
                          &   $w_\mathrm{high}$ &   $0.036\pm0.067$ &            $0.0\pm0.0$ \\
                          &  $w_\mathrm{incl.}$ &   $0.015\pm0.046$ &            $0.0\pm0.0$ \\
\bottomrule
\end{tabular}
\end{table}


==> supplemental_material.tex <==
In Fig.~\ref{fig:equivalence}, we illustrate the equivalence between the definitions of \sthree, \sfive, \sseven, and \snine{} found in Ref.~\cite{bhattacharya} and the one-dimensional reinterpretation described in the text. In Table~\ref{tab:results_sm}, we show the results for all $\mathcal{A}$ and \deltaA{} observables in the three $w$ ranges, with uncertainties classified by source in Table~\ref{tab:systematics_sm}. We show the statistical and systematic covariance matrices in Figs.~\ref{fig:cov_stats} and \ref{fig:cov_syst}, respectively. 

% Without this, latex insists on putting figs above the section header. Using flafter does the same thing as this. 
\clearpage




\begin{figure}
  \centering
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[scale=.8]{figures/tikz/s3.pdf}
    \tikz[scale=0.8]{
      \draw[draw=none] (0, -1) rectangle (0.2, 1.2) node [pos=.5] {\LARGE\(\equiv\)};
    }
    \includegraphics[scale=.8]{figures/tikz/s3-transformed.pdf}
    \captionsetup{justification=centering}
    \caption{\sthree\label{fig:s3}}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[scale=.8]{figures/tikz/s5.pdf}
    \tikz[scale=0.8]{
      \draw[draw=none] (0, -2) rectangle (0.2, 1.2) node [pos=.5] {\LARGE\(\equiv\)};
    }
    \includegraphics[scale=.8]{figures/tikz/s5-transformed.pdf}
    \captionsetup{justification=centering}
    \caption{\sfive\label{fig:s5}}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[scale=.8]{figures/tikz/s7.pdf}
    \tikz[scale=0.8]{
      \draw[draw=none] (0, -2) rectangle (0.2, 1.2) node [pos=.5] {\LARGE\(\equiv\)};
    }
    \includegraphics[scale=.8]{figures/tikz/s7-transformed.pdf}
    \captionsetup{justification=centering}
    \caption{\sseven\label{fig:s7}}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[scale=.8]{figures/tikz/s9.pdf}
    \tikz[scale=0.8]{
      \draw[draw=none] (0, -1) rectangle (0.2, 1.2) node [pos=.5] {\LARGE\(\equiv\)};
    }
    \includegraphics[scale=.8]{figures/tikz/s9-transformed.pdf}
    \captionsetup{justification=centering}
    \caption{\snine\label{fig:s9}}
  \end{subfigure}
  \captionsetup{justification=centering}
  %\caption{An illustration of the equivalence between the asymmetry categories of Ref.~\cite{bhattacharya} and our one-dimensionalized categories.}
  \caption{An illustration of the equivalence between the two-dimensional asymmetry categories of Ref.~\cite{bhattacharya} and our one-dimensional categories. All asymmetry variables are defined as normalized differences between yields of + (blue) and - (yellow) regions of their respective angular variable(s).}
  \label{fig:equivalence}
\end{figure}

\input{afb_results_table_sm.tex}
\input{afb_syst_table_sm.tex}

\begin{figure*}[b]
  \centering
    \includegraphics[width=\textwidth]{figures/angular_obs_boostrap_cov_prl}

  \caption{Statistical covariance matrix determined by sampling experimental data with replacement.}
  \label{fig:cov_stats}
\end{figure*}

\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{figures/syst_cov_matrix_prl}

  \caption{Systematic covariance matrix, using the same color scale as Fig.~\ref{fig:cov_stats} in order to illustrate the relative contributions to the total covariance matrix. }
  \label{fig:cov_syst}
\end{figure*}

==> title.tex <==
% WRITE THE TITLE IN THIS FILE.
